Stable Boundary Layers with Subsidence: Scaling and Similarity of the Truly Steady State

The stable boundary layer (SBL) subjected to large-scale subsidence is studied through large-eddy simulations (LESs) with fixed surface temperature and a linear subsidence velocity profile. These boundary layers reach a truly steady state, where thermal equilibrium is established by a balance between surface cooling and subsidence-induced heating. We identify three governing dimensionless groups by scaling the governing equations with the geostrophic wind and Coriolis frequency, and systematically investigate the impact of these external parameters on global flow properties and mean profiles in the steady state. The SBL depth, low-level jet, and the magnitude of the turbulent momentum flux are reduced when the subsidence rate or Buoyancy number increases, while surface heat flux is enhanced. The shape of normalized mean profiles of temperature and heat flux is mainly determined by the subsidence rate, while they collapse for varying buoyancy and surface Rossby numbers. We develop empirical correlations for the stability parameter $h_{\theta}/L_O$ and a thermal shape factor, and propose a new unidirectional geostrophic drag law, to form a closed set of equations that estimates relevant flow properties from external parameters. The estimation errors compared to the LES data are less than 5% for friction velocity and surface heat flux, and at most 10% for the SBL depth $h_{\theta}$. Within the surface layer, dimensionless velocity and temperature gradients in the steady SBL with subsidence show acceptable agreement to Monin-Obukhov similarity theory, while the collapse is improved when a recently proposed mixed scaling parameter, that includes $h_{\theta}/L_O$, is used.

==> Content/introduction_old.tex <==
\section{Introduction}
\label{sec:intro}
Stably stratified boundary layers generally occur when warm fluid flows over a colder surface. The atmospheric boundary layer (ABL), is typically stably stratified at night, or in summertime over sea \citep{Stull1988, Wyngaard2010}. Understanding the stable boundary layer (SBL) can be viewed as one of the key challenges in the atmospheric and environmental sciences, and is relevant to the renewable energy sector, air quality and pollutant dispersion, numerical weather prediction (NWP) and climate modelling. Idealized numerical simulations play an important role in investigations of SBLs, in particular Large-Eddy Simulations (LES) and Direct Numerical Simulations (DNS) \citep{Stoll2020}. In a vast amount of these numerical studies, the focus is on the physics of stratified turbulence, or its parametrization in LES or large-scale models \citep{Nieuwstadt2005, Sullivan2016a, Dai2021, Maronga2022}. Other works examine the interaction between the SBL and some additional `complexity', for example wind farms \citep{Allaerts2018, Strickland2022a}, non-uniform surface roughness \citep{Lee2020, Forooghi2020}, or surface temperature heterogeneity \citep{Stoll2009, Mironov2016}.

In the canonical, idealized simulation setup utilized for stable boundary layers, the surface boundary condition for temperature involves either a prescribed heat flux \citep[e.g.][]{Nieuwstadt2005, Flores2011, Gohari2017}, fixed temperature \citep{Ansorge2014, Shah2014}, constant cooling rate \citep[e.g.][]{Beare2006, Huang2013, Narasimhan2023} or a combination thereof \citep{Gohari2018}. One thing that all the above-mentioned studies have in common, is that the simulations never reach a perfectly stationary state, where both the turbulent and thermal energy of the system are in (statistical) equilibrium. In case of cooling rate or heat flux boundary conditions, the surface temperature keeps decreasing, whereas the surface heat flux keeps changing when the surface temperature is held constant. In both scenarios, the domain-averaged temperature continuously declines (as further explained in the next section and equation \eqref{eq:balance}).  .

This non-stationarity is obviously no problem for research that aims to investigate flow dynamics, such as the transition from a (conventionally) neutral to a stable boundary layer \citep{Allaerts2018, Gohari2018}. Besides, many studies employ the fact that the SBL often reaches a ``quasi-steady'' state after some time, in which the mean profiles of velocity and turbulence statistics remain constant while only the temperature profile keeps changing. In numerous applications however, it is desired to have long averaging times under truly stationary conditions, without any transient effects, to permit more systematic analysis and comparison of multiple different simulations.
 
For example, the study of large-scale secondary motions that can be induced by heterogeneous surface roughness or temperatures, requires long averaging times \citep{Bon2022, Castro2021, Schafer2022a, Amarloo2022a}. When employing LES for a systematic analysis of the effects of large wind farms on atmospheric heat fluxes, examination of stationary statistics considerably simplifies understanding \citep{Sescu2014}. Moreover, when assessing the sensitivity of an LES code to the grid spacing or the subgrid-scale model in an SBL simulation, the constantly decreasing surface temperature prevents using long averaging times \citep{Maronga2022}.

In the present paper, we demonstrate how adding a constant (in time) subsidence term to the temperature equation is a simple and physically elegant way to make LES of the SBL reach a thermal equilibrium and thus a truly stationary state. Moreover, we systematically investigate how this equilibrium state depends on external parameters such as surface temperature, subsidence rate and surface roughness.  Although our simulation set-up is strongly idealized, the subsidence rate and other flow parameters are actually realistic in an ABL. We should emphasize that we are not the first to investigate the effect of subsidence on an SBL or apply it to reach a truly steady state, but a systematic analysis  of the full parameter space that plays a role in the simplified SBL with subsidence has not been performed before.

Several previous studies have already shown that even weak subsiding motions can have large implications on the SBL, particularly in the polar regions. Based on data from the Surface Heat Budget of the Arctic Ocean (SHEBA) field experiment, \cite{Mirocha2005a} suggest that a significant portion of the heat lost to the surface by turbulent heat flux is balanced by heating near the ABL-top due to the interaction of subsiding motions with the strong overlying temperature inversion. Later, \cite{Mirocha2010} showed with LES that the addition of subsidence reduces the vertical momentum fluxes while enhancing vertical heat flux, increases temperature gradients, and limits the growth of the boundary layer, leading to a ``nearly  steady boundary layer behaviour during periods of constant forcing''. Moreover, they state that subsidence affects other physical processes in the SBL, such as the low-level cloud field and growth/ablation of the snow/ice pack due to changes in surface heat flux.

More recently, \cite{VanderLinden2019} performed centimetre-scale LESs of a weakly and very stable boundary layer and compared results to observational data from the Dome C station on the Antarctic Plateau, where the absence of the diurnal cycle during the Antarctic winter facilitated the examination of a long-lived steady stable boundary layer. They concluded that the inclusion of subsidence can result in thermal equilibrium of the SBL, as the turbulent cooling towards the surface is balanced by the heating due to subsidence. However, although these LES studies confirm that subsidence is an important external scaling parameter for the (nearly) steady SBL, they also establish that further simulation and theoretical work is needed to fully understand the complex relationship between subsidence, ABL height, vertical heat and momentum fluxes, velocity and temperature profiles. One aim of the present study is to (partly) fill this gap, by analysing a broad set of LES cases where the subsidence rate, surface temperature and roughness are varied.

Other studies have investigated the impact of subsidence in contexts beyond stable boundary layers. In LES of cloud-topped marine boundary layers, subsidence can also lead to steady-state \citep{Chung2012, Bellon2012}. However, the resulting energy balance is then more complicated than in the present case due to radiation and humidity effects. \cite{Kurowski2020} showed that even weak, finite-time perturbations of horizontal convergence can have a strong impact on shallow convection in cloud-topped boundary layers. \cite{Mazzitelli2014} investigated effects of subsidence in near-neutral and unstable boundary layers.
In LES of very large wind farms under varying atmospheric conditions, \cite{Maas2022} apply subsidence to prevent their convective boundary layer from growing, while stating that reaching equilibrium in an SBL is ``not as simple''. Earlier, \cite{Sescu2014} developed a control algorithm to reach a statistically stationary state in LES of thermally stratified boundary layers, by adding a heat source in the free atmosphere above the turbulent boundary layer based on a proportional-integral (PI) controller. This is however a less physical solution, and seems not to have been applied in later studies (?). 

In the present paper, we present and analyze results of a set of LESs of stable boundary layers, where the addition of subsidence heating ensures that thermal equilibrium is reached. Apart from the subsidence term, the simulation setup is loosely based on the Global Energy and Water Cycle Experiment Atmospheric Boundary Layer Study 1 (GABLS1, \cite{Beare2006}). This is probably the most widely studied and well-documented setup for LES of SBLs, and is up till now still used as a reference case to e.g. validate new LES codes \citep{VanHeerwaarden2017}, evaluate new subgrid models or surface parametrizations \citep{Dai2021, Maronga2020} and assess grid-size sensitivity of LES \cite{Maronga2022}. Besides, many LES studies that investigate stably stratified turbulence use a slightly modified configuration to study effects of increasing stability \cite{Sullivan2016a}, heterogeneous surface temperatures \cite{Stoll2009, Mironov2016}, or interaction between the SBL and a wind-farm \citep{Allaerts2018}.



In section \ref{sec:theory_methods} we first discuss some background theory and derive useful relations that will be used in the analysis of the results. Further, the numerical methodology is described and the case setup outlined. In sectrion \ref{sec:results} we first discuss the general effect of the input parameters on mean profiles, followed by analysis of correlations between mean flow variables...?


apply subsidence to reach a truly stationary stable boundary layer. We investigate implications and look for scaling and similarity. Can be useful for defining a canonical reference case for stable boundary layers that is not transient, e.g. to enable grid-size sensitivity studies and SGS models in a more formal systematic way.
Fu

%``Even if the real-world stratified ABL is most of the time evolving in time, the idealized behaviour of statistical stationarity is useful to analyze and understand generic, canonical behaviour. For example, this is often desired when one carries out LES of the ABL and studies the interactions between large wind farms and the thermally stratified ABL. Specifically, such conditions are desirable in order to make meaningful comparisons between the expected behaviour of the ABL with and without wind turbines. Together, these two control schemes enable very long-time simulations of thermally stratified heated or cooled boundary layers displaying fully stationary distributions of mean velocity and temperature.'' And heterogeneity! This canonical steady-state problem permits a systematic quantative comparison between different codes, sgs models etc. 


%Related to GABLS:
%\cite{Dai2021}
%\cite{Maronga2020} also have a neutral layer above the boundary layer, where they observe inertial oscillations. ``As the surface was continuously cooled, no true steady temperature state could be achieved, but we observed convergence of time series (e.g., friction velocity) after about 16h''
%\cite{Maronga2022} point out that flow GABLS case is still evolving in hour 9, particularly affected by inertial oscillation. Therefore, they run for 36 hours. ``However, as the temperature continues to drop, using longer averaging periods would result in substantial changes in thermodynamic quantities. '' 







